3D Shape Induction from 2D Views of Multiple Objects

In this paper we investigate the problem of inducing a distribution over three-dimensional structures given two-dimensional views of multiple objects taken from unknown viewpoints. Our approach called "projective generative adversarial networks" (PrGANs) trains a deep generative model of 3D shapes whose projections match the distributions of the input 2D views. The addition of a projection module allows us to infer the underlying 3D shape distribution without using any 3D, viewpoint information, or annotation during the learning phase. We show that our approach produces 3D shapes of comparable quality to GANs trained on 3D data for a number of shape categories including chairs, airplanes, and cars. Experiments also show that the disentangled representation of 2D shapes into geometry and viewpoint leads to a good generative model of 2D shapes. The key advantage is that our model allows us to predict 3D, viewpoint, and generate novel views from an input image in a completely unsupervised manner.

==> conclusion.tex <==
\section{Conclusion and Future Work}\label{s:conclusion}
We proposed a 


%\paragraph{Limitations.} low resolution; objects with concave interior; shading and texture information, lack of geometric details (how to enhance geometric details?)


==> exp2.tex <==
\section{Experiments}\label{s:experiments}


In this section we describe the set of experiments to evaluate our method
and to demonstrate the extension of its capabilities.
First, we show the effectiveness of our method as both 2D and 3D shape generators.
To this end, we compare our model with a traditional GAN for image generation and a
GAN for 3D shapes.
We present quantitative and qualitative results.
Second, we demonstrate that our method is able to induce 3D shapes from
unlabelled images even when there is only a single view per object.
Third, we present 3D shapes induced by our model from a variety of categories such as airplanes, cars, chairs, motorbikes, and vases. Using the same architecture, we show how our model is able to induce coherent 3D shapes when the training data contains images mixed from multiple categories.
Finally, we show applications of our method in predicting 3D shape from a novel 2D shape, and performing shape interpolation.

\begin{figure}[t]
\setlength{\tabcolsep}{0pt}
\begin{tabular}{cccc}
\includegraphics[width=.25\linewidth]{fig/comparison/2dgan0.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/2dgan3.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/2dgan5.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/2dgan7.png} \\
\multicolumn{4}{c}{(a) Results from 2D-GAN.} \vspace{4pt}\\
\includegraphics[width=.25\linewidth]{fig/comparison/pr2dgan4.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/pr2dgan5.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/pr2dgan6.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/pr2dgan3.png} \\
\multicolumn{4}{c}{(a) Results from PrGAN.} \vspace{4pt}
\end{tabular}
\caption{\label{fig:validation2D} Comparision between 2D-GAN~\cite{} and our PrGAN model for image generation on the chairs dataset. Refer to Fig.~\ref{fig:generate-shapes} third row, left column for samples of the input data.}
\end{figure}

\paragraph{Input data.} We generate training images synthetically using several categories of 3D shapes available in the
ModelNet~\cite{} and ShapeNet~\cite{} databases. Each category contains a few hundred to thousand shapes. We render each
shape from 8 evenly spaced viewing angles with orthographic projection to produce binary images. To reduce aliasing, we
render each image at $64\times64$ resolution and downsample to $32\times32$. We have found that this generally improves
the results. Using synthetic data allows us to easily perform controlled experiments to analyze our method. 
It is also possible to use real images downloaded from a search engine as discussed in Section \ref{s:discussion}.

\paragraph{Validation.}
We quantitatively evaluate our model by comparing its ability to generate
2D and 3D shapes.
In order to do that, we use 2D image GAN similar to DCGAN~\cite{radford2015unsupervised} and a 3D-GAN
similar to the one presented at \cite{wu2016learning}.
We will refer to them as 2D-GAN and 3D-GAN, respectively.
The 2D-GAN has the same discriminator architecture as the PrGAN, but the generator contains a sequence of 2D transposed convolutions instead of 3D ones, and
the projection module is removed.
The 3D-GAN has a discriminator with 3D convolutions instead of 3D ones.
The 3D-GAN generator is the same of the PrGAN, but without the projection module.

%Maybe this should be in the method section?
The models used in this experiment are chairs from ModelNet dataset~\cite{wu20153d}.
From those models, we create two sets of training data: voxel grids and images.
The voxel grids are generated by densely sampling the surface and inside of each mesh, and binning the sample points into $32\times32\times32$ 
grid.
A value 1 is assigned to any voxel that contains at least one sample point, and 0 otherwise.
Notice that the voxel grids are only used to train the 3D-GAN, while the images are used to train the 2D-GAN and our PrGAN.
%The images are created using the same models and rendered a binary images.
% Regions that contain the model are white, and regions that do not contain the model are black.
%For each chair model, we create 8 different images by uniformly
%rotating the model around the vertical axis.
%Also, we observed that the performances of the 2D-GAN and the PrGAN are enhanced if the images
%are rendered in $64\times64$ and downsampled to $32\times32$.
N%otice that the data used to train the PrGAN consists of images, but the method is able to learn a generative model for 3D shapes from those images, which makes it comparable to the 3D-GAN.

\begin{figure}[t]
\setlength{\tabcolsep}{0pt}
\begin{tabular}{cccc}
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan8.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan9.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan10.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan11.png} \\
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan12.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan13.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan14.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan15.png} \\
\multicolumn{4}{c}{(a) Results from 3D-GAN.} \vspace{4pt}\\
\includegraphics[width=.25\linewidth]{fig/comparison/prgan0.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/prgan1.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/prgan2.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/prgan3.png} \\
\includegraphics[width=.25\linewidth]{fig/comparison/prgan4.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/prgan5.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/prgan6.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/prgan7.png} \\
\multicolumn{4}{c}{(a) Results from PrGAN.} \vspace{4pt}\\
\end{tabular}
\caption{\label{fig:validation3D} Comparison between 3D-GAN~\cite{} and our PrGAN for 3D shape generation. The 3D-GAN is trained on 3D voxel representation of the chair models, and the PrGAN is trained on images of the chair models (refer to Fig.~\ref{fig:generate-shapes} third row).}
\end{figure}

Our quantitative evaluation is done by taking the Maximum Mean Discrepancy (MMD)~\cite{gretton2006kernel} 
between the data created by the generative models and the training data.
We use a kernel bandwidth of $10^{-3}$ for images and $10^{-2}$ for voxel grids.
The training data consists of 989 voxel grids and 7912 images.
To compute the MMD, we draw 128 random data points from each one of the generative models.
The distance metric between the data points is the hamming distance divided by the dimensionality of the data.
Because the data represent the continuous occupancy values, we binaritize them by using a threshold of $0.001$ for images or voxels created
by PrGAN, and $0.1$ for voxels created by the 3D-GAN.

\begin{figure}[t]
\includegraphics[width=0.95\linewidth]{fig/varying_views.png}
\caption{\label{fig:varying_views} Shapes generated from PrGAN by varying the number of views per object in the training data. From the top row to the bottom row, the number of views per object in the training set are 1, 2, 4, and 8 respectively.}
\end{figure}

Results show that for 2D-GAN, the MMD between the generated images and the training data is 90.13. For PrGAn, the MMD is 88.31, which is slightly better quantitatively than 2D-GAN. Fig.~\ref{fig:validation2D} shows a qualitative comparison. The results are visually very similar. For 3D-GAN, the MMD between the generated voxel grids and the training voxel grids is 347.55. For PrGAN, the MMD is 442.98, which is worse compared to 3D-GAN. This is not surprising as 3D-GAN is trained on 3D data, while PrGAN is trained on the image views only. Fig.~\ref{fig:validation3d} presents a qualitative comparison. In general PrGAN has trouble generating intrior structures because the training images are binary, carries no shading information, and are taken from a limited set of viewing angles. Nonetheless, it learns to generate exterior structures reasonably well.

\paragraph{Varying the number of views per model.} In the default setting, our training data consists of 8 views per object. Here we study the ability of our method in the more challenging case where the training data contains fewer number of views per object. To do so, we generate a new training set that contains only 1 randomly chosen view per object and use it to train PrGAN. We then repeat the experiments for 2 randomly chosen views per object, and also 4. The results are shown in Fig.~\ref{fig:varying_views}. The 3D shapes that PrGAN learns becomes increasingly better as the number of views increases. Even in the single view per object case, our method is able to induce reasonable shapes. 

\begin{figure}[t]
\includegraphics[width=0.95\linewidth]{fig/shape_prediction/sp.png}
\caption{\label{fig:sp} Shapes infered by a single image using the encoding network.}
\end{figure}

\rui{should we explain the assumption about the distribution of the views?}
%Our standard experimental setup uses eight images taken from the same eight different viewpoints.
%An interesting question is to assess the ability of the method to learn
%how to generate shapes when the one or more of the views is not accessible.
%To evaluate this issue, we create three different datasets.
%The first one, contains only one randomly selected image from the eight previously available.
%The second and third dataset contain two and four images.
%As we can see in Fig.~\ref{fig:varying_views}, our method is able to induce
%reasonable shapes even when a single view is available.
%However, the quality improves as the number of available views increases.


\paragraph{Visualizations across categories.} Our method is able to generate 3D shapes for a wide range of categories. Fig.~\ref{fig:generate-shapes} show a gallery of results, including airplanes, car, chairs, vases, motorbikes. For each category we show 64 randomly sampled training images, 64 generated images from PrGAN, and renderings of 128 generated 3D shapes (produced by randomly sampling the 200-d input vector of the generator). 
%shows the input images and sampled models and views of airplanes, chairs, vases, and motorbikes.
One remarkable property is that the generator produces 3D shapes in a consistent horizontal and vertical axes, even though the training data is only consistently oriented along the vertical axis. Our hypothesis for this is that the generator finds it more efficient to generate shapes in a consistent manner by sharing parts across models. Fig.~\ref{fig:example-samples} shows selected examples from Fig.~\ref{fig:generate-shapes} that demonstrates the quality and diversity of the generated shapes. 

The last row in Fig.~\ref{fig:generate-shapes} shows an example of a 'mixed' category, where the training images combine the three categories of airplane, car, and motorbike. The same PrGAN network is used to learn the shape distributions. Results show that PrGAN learns to represent all three categories well, without any additional supervision.

%Here we investigate if a single generative model can generate shapes across multiple categories without any additional supervision. For this experiment we combine views of models across airplanes, motorbikes, and cars and provide them as input to the learning algorithm. The bottom row in Figure~\ref{fig:generate-shapes} shows the results. 


\begin{figure}[t]
\setlength{\tabcolsep}{0pt}
\begin{tabular}{cccccccc}
\includegraphics[width=.125\linewidth]{fig/interpolation/ap0.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ap1.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ap2.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ap3.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ap4.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ap5.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ap6.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ap7.png} \\
\includegraphics[width=.125\linewidth]{fig/interpolation/ch0.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ch1.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ch2.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ch3.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ch4.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ch5.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ch6.png} &
\includegraphics[width=.125\linewidth]{fig/interpolation/ch7.png} \\
\end{tabular}
\caption{\label{fig:interp} Interpolation between two different encodings. Top row shows a model trained on airplanes.
Borrom row shows a model trained on chairs.}
\end{figure}

\paragraph{Shape interpolation.}
Once the generator is trained, any value of $z$ supposedly generates a plausible 3D shape, hence $z$ represents a 3D shape manifold. Similar to previous work, we can interpolate between 3D shapes by interpolating their $z$ code. Fig.~\ref{fig:interp} shows the results by linearly interpolating the $z$ code between two generated airplane shapes.
%Such properties have been demonstrated for other deep generative models and we show that
%the generator learned by our method works in the same way.
%Our experiment consists of training our model with the airplane dataset from ShapeNet~\cite{}, selecting
%the encodings of two different shapes and interpolating them.
%As we can see in 

\paragraph{Unsupervised shape and viewpoint prediction.}
Our method is also able to handle unsupervised prediction of shapes in 2D images.
Once we train our model, we have a 3D shape generator that is capable of creating shapes from
a set of encodings $z \in \mathbb{R}^{201}$.
Thus, our goal is to predict the encoding of the object that is displayed in the image.
We do this by training a neural network with images created by the previously trained PrGAN.
In other words, we create a training set that consists of images synthesized by the PrGAN and
the encodings that generated them.
The neural network is a fully connected one, with 2 hidden layers, each one with 512 neurons.
The input of the network is an image and the output is an encoding.
The last number of $z$ describes the view and the other 200 describe the shape.
We use these 200 values to retrieve the shape present in the image.
The network is trained with images created by the PrGAN, but we present the results of the network
using the original dataset images as input in Figure \ref{fig:sp}.
This whole process constitutes a completely unsupervised approach to
creating a model to infer a 3D shape from a single image.

\begin{figure*}
  \newcommand{\fh}{0.19\linewidth}
  \begin{center}
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{ccc}
    \textbf{Input} & \textbf{Generated images} & \textbf{Generated shapes} \\
    \includegraphics[height=\fh]{fig/airplane/samples.png} & 
    \includegraphics[height=\fh]{fig/airplane/100.png} & 
    \includegraphics[height=\fh]{fig/airplane/output.png} \\
    \includegraphics[height=\fh]{fig/car/samples.png} & 
    \includegraphics[height=\fh]{fig/car/600.png} & 
    \includegraphics[height=\fh]{fig/car/output.png} \\
    \includegraphics[height=\fh]{fig/chair/samples.png} & 
    \includegraphics[height=\fh]{fig/chair/550.png} & 
    \includegraphics[height=\fh]{fig/chair/output.png} \\
    \includegraphics[height=\fh]{fig/vase/samples.png} & 
    \includegraphics[height=\fh]{fig/vase/450.png} & 
    \includegraphics[height=\fh]{fig/vase/output.png} \\
    \includegraphics[height=\fh]{fig/bike/samples.png} & 
    \includegraphics[height=\fh]{fig/bike/300.png} & 
    \includegraphics[height=\fh]{fig/bike/output.png} \\
    \includegraphics[height=\fh]{fig/mix/samples.png} & 
    \includegraphics[height=\fh]{fig/mix/0.png} & 
    \includegraphics[height=\fh]{fig/mix/output.png} \\
  \end{tabular}
  \end{center}
  \vspace{-6pt}
  \caption{\label{fig:generate-shapes} Results for 3D shape induction using PrGANs. From top to bottom we show results for airplane, car, chair, vase, motorbike, and a 'mixed' category obtained by combining training images from airplane, car, and motorbike. At each row, we show on the left 64 randomly sampled images from the input data to the algorithm, on the right 128 sampled 3D shapes from PrGAN, and in the middle 64 sampled images after the projection module is applied to the generated 3D shapes. The model is able to induce a rich 3D shape distribution for each category. The mixed-category produces reasonable 3D shapes across all three combined categories. Zoom in to see details.}
\end{figure*}

\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{0pt}
\begin{tabular}{cccccccc}
\includegraphics[width=.125\linewidth]{fig/airplane/sel0009.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0012.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0007.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0003.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0002.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0004.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0006.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0008.png} \\
\includegraphics[width=.125\linewidth]{fig/car/sel0010.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0005.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0001.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0004.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0002.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0006.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0007.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0008.png} \\
\includegraphics[width=.125\linewidth]{fig/vase/sel0013.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0003.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0011.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0015.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0001.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0014.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0016.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0007.png} \\
\includegraphics[width=.125\linewidth]{fig/bike/sel0006.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0005.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0008.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0004.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0007.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0003.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0002.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0001.png} 
\end{tabular}
\caption{\label{fig:example-samples} A variety of 3D shapes generated by PrGAN trained on 2D views of (from the top row to the bottom row) airplanes, cars, vases, and bikes. These examples are chosen from the gallery in Fig.~\ref{fig:generate-shapes} and demonstrate the quality and diversity of the generated shapes.}\end{figure*}


==> exps2.tex <==
\section{Experiments}\label{s:experiments}



In this section we describe the set of experiments to evaluate our method
and to demonstrate the extension of its capabilities.
First, we show the effectiveness of our method as both 2D image and 3D shape generator.
To this end, we compare our model with a traditional GAN for image generation and a
GAN for 3D shapes.
We present quantitative and qualitative results.
Second, we demonstrate that our method is able to induce 3D shapes from
unlabelled images even when there is only a single view per object.
Third, using the same architecture, we show how our model is able to
induce coherent 3D shapes when the training data contains images of
different categories, like chairs and cars.
Finally, we present 3D shapes induced by our model from a broad range of categories like
airplanes, cars, chairs, beds and vases.

\begin{figure}[t]
\setlength{\tabcolsep}{0pt}
\begin{tabular}{cccc}
\includegraphics[width=.25\linewidth]{fig/comparison/2dgan0.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/2dgan3.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/2dgan5.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/2dgan7.png} \\
\multicolumn{4}{c}{(a) Results from 2D-GAN.} \vspace{4pt}\\
\includegraphics[width=.25\linewidth]{fig/comparison/pr2dgan4.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/pr2dgan5.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/pr2dgan6.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/pr2dgan3.png} \\
\multicolumn{4}{c}{(a) Results from PrGAN.} \vspace{4pt}
\end{tabular}
\caption{\label{fig:validation} Comparision between 2D-GAN~\cite{} and our PrGAN model for image generation on the chairs dataset. Refer to Fig.~\ref{fig:generate-shapes} third row, left column for samples of the input data.}
\end{figure}

\paragraph{Input data.} explain the source of input data, how many models, 8 views per model, roughly how many images.

\paragraph{Validation.}
We quantitatively evaluate our model by comparing its ability to generate
images and 3D shapes.
In order to do that, we use 2D image GAN similar to DCGAN~\cite{radford2015unsupervised} and a 3D-GAN
similar to the one presented at \cite{wu2016learning}.
We will refer to them as 2D-GAN and 3D-GAN, respectively.
The 2D-GAN has the same discriminator architecture as the PrGAN.
But, the generator contains a sequence of 2D transposed convolutions instead of 3D ones and
the projection module is removed.
On the other hand, the 3D-GAN has a discriminator with 3D convolutions instead of 3D ones.
The 3D-GAN generator is the same of the PrGAN, but without the projection module.

%Maybe this should be in the method section?
The models used in this experiment are chair models taken from ModelNet dataset~\cite{wu20153d}.
From those models, we create two sets of training data: voxel grids and images.
The voxel grids are computed by sampling points on the surface and inside of the meshes.
Those points are scaled and translated to fit inside $32\times32\times32$ voxel
grid.
The final voxel grid is computed by assigning a value 1 to any voxel that contains
at least one point and 0, otherwise.
Notice that the voxel grids are only used to train the 3D-GAN.
The images are created using the same models and rendered a binary images.
Regions that contain the model are white, and regions that do not contain the model
are black.
For each chair model, we create 8 different images by uniformly
rotating the model around the vertical axis.
Also, we observed that the performances of the 2D-GAN and the PrGAN are enhanced if the images
are rendered in $64\times64$ and downsampled to $32\times32$.
Notice that the data used to train the PrGAN consists of images, but the method
is able to learn a generative model for 3D shapes from those images, which makes
it comparable to the 3D-GAN.

\begin{figure}[t]
\setlength{\tabcolsep}{0pt}
\begin{tabular}{cccc}
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan0.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan1.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan2.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan3.png} \\
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan4.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan5.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan6.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/3dgan7.png} \\
\multicolumn{4}{c}{(a) Results from 3D-GAN.} \vspace{4pt}\\
\includegraphics[width=.25\linewidth]{fig/comparison/prgan0.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/prgan1.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/prgan2.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/prgan3.png} \\
\includegraphics[width=.25\linewidth]{fig/comparison/prgan4.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/prgan5.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/prgan6.png} &
\includegraphics[width=.25\linewidth]{fig/comparison/prgan7.png} \\
\multicolumn{4}{c}{(a) Results from PrGAN.} \vspace{4pt}\\
\end{tabular}
\caption{\label{fig:validation} Comparison between 3D-GAN~\cite{} and our PrGAN for 3D shape generation. The 3D-GAN is trained on 3D voxel representation of the chair models, and the PrGAN is trained on images of the chair models (refer to Fig.~\ref{fig:generate-shapes} third row).}
\end{figure}

Our quantitative evaluation is done by taking the Maximum Mean Discrepancy (MMD)~\cite{gretton2006kernel} 
between the data created by the generative models and the training data.
We use a kernel bandwidth of $10^{-3}$ for images and $10^{-2}$ for voxel grids.
The training data consists of 989 voxel grids and 7912 images.
To compute the MMD, we use 128 data points from each one of the generative models.
The distance between the data points is the hamming distance divided by the dimensionality of the data.
However, we to binarize the data created by the generators.
This is done by setting to 1 any value bigger then $0.001$ in the images or in voxel grids created
by PrGAN.
For the voxel grids created by the 3D-GAN the threshold is $0.1$.
The difference is a consequence of the fact that the training images are not binary
due to the downsampling step in their creation.
The MMD between the images generated by the 2D-GAN and the training data is 90.13.
When using the images generated by the PrGAN, the distance is 88.31.
The MMD between the voxel grids generated by the 3D-GAN and the training data is 347.55.
When using the voxel grids generated by the PrGAN, the distance is 442.98.
Figure~\ref{fig:validation} presents a qualitative comparison of the generated data.

\paragraph{Varying number of views per model}
Our standard experimental setup uses eight images taken from the same eight different viewpoints.
An interesting question is to assess the ability of the method to learn
how to generate shapes when the one or more of the views is not accessible.
To evaluate this issue, we create three different datasets.
The first one, contains only one randomly selected image from the eight previously available.
The second and third dataset contain two and four images.
As we can see in Fig.~\ref{fig:varying_views}, our method is able to induce
reasonable shapes even when a single view is available.
However, the quality improves as the number of available views increases.

\begin{figure}[t]
\includegraphics[width=0.95\linewidth]{fig/varying_views.png}
\caption{\label{fig:varying_views} Shapes generated varying the number of available images per object.
Top row: one image per object. Second row: two images per object. Third row: four images
per object. Bottom row: full dataset (eight images per object).}
\end{figure}

\begin{figure}[t]
\includegraphics[width=0.95\linewidth]{fig/shape_prediction/sp.png}
\caption{\label{fig:sp} Shapes infered by a single image using the encoding network.}
\end{figure}

\paragraph{Visualizations across categories.} Our model is able to generate 3D shapes for a wide range of categories. Fig.~\ref{fig:generate-shapes} shows the input images and sampled models and views of airplanes, chairs, vases, and motorbikes. One remarkable property is that the generator generates the 3D shapes in a consistent horizontal and vertical orientation even though the dataset is only consistently oriented along the vertical axis. Our hypothesis for this is that the generator finds it more efficient to generate shapes in a consistent manner by sharing parts across models.

\begin{figure*}
  \newcommand{\fh}{0.19\linewidth}
  \begin{center}
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{ccc}
    \textbf{Input} & \textbf{Generated images} & \textbf{Generated shapes} \\
    \includegraphics[height=\fh]{fig/airplane/samples.png} & 
    \includegraphics[height=\fh]{fig/airplane/100.png} & 
    \includegraphics[height=\fh]{fig/airplane/output.png} \\
    \includegraphics[height=\fh]{fig/car/samples.png} & 
    \includegraphics[height=\fh]{fig/car/600.png} & 
    \includegraphics[height=\fh]{fig/car/output.png} \\
    \includegraphics[height=\fh]{fig/chair/samples.png} & 
    \includegraphics[height=\fh]{fig/chair/550.png} & 
    \includegraphics[height=\fh]{fig/chair/output.png} \\
    \includegraphics[height=\fh]{fig/vase/samples.png} & 
    \includegraphics[height=\fh]{fig/vase/450.png} & 
    \includegraphics[height=\fh]{fig/vase/output.png} \\
    \includegraphics[height=\fh]{fig/bike/samples.png} & 
    \includegraphics[height=\fh]{fig/bike/300.png} & 
    \includegraphics[height=\fh]{fig/bike/output.png} \\
    \includegraphics[height=\fh]{fig/mix/samples.png} & 
    \includegraphics[height=\fh]{fig/mix/0.png} & 
    \includegraphics[height=\fh]{fig/mix/output.png} \\
  \end{tabular}
  \end{center}
  \vspace{-6pt}
  \caption{\label{fig:generate-shapes} Results for 3D shape induction using PrGANs. From top to bottom we show results for airplane, car, chair, vase, motorbike, and a 'mixed' category obtained by combining training images from airplane, car, and motorbike. At each row, we show on the left 64 randomly sampled images from the input data to the algorithm, on the right 128 sampled 3D shapes from PrGAN, and in the middle 64 sampled images after the projection module is applied to the generated 3D shapes. The model is able to induce a rich 3D shape distribution for each category. The mixed-category produces reasonable 3D shapes across all three combined categories. Zoom in to see details.}
\end{figure*}


\paragraph{Multi-category model} Here we investigate if a single generative model can generate shapes across multiple categories without any additional supervision. For this experiment we combine views of models across airplanes, motorbikes, and cars and provide them as input to the learning algorithm. The bottom row in Figure~\ref{fig:generate-shapes} shows the results. 


\paragraph{Shape interpolation.}
Once we have the generator trained, any value of $z$ describes a 3D shape.
We can think of $z$ as a 3D shape manifold.
Such properties have been demonstrated for other deep generative models and we show that
the generator learned by our method works in the same way.
Our experiment consists of training our model with the airplane dataset from ShapeNet~\cite{}, selecting
the encodings of two different shapes and interpolating them.
As we can see in Figure \ref{fig:interp}, interpolation in the encoding space 
translates to a interpolation in the shape space as we can see in
\begin{figure}[t]
\includegraphics[width=0.95\linewidth]{fig/interpolation.png}
\caption{\label{fig:interp} Interpolation between two different encodings in a model trained on airplanes.}
\end{figure}

\paragraph{Unsupervised shape and viewpoint prediction.}
Our method is also able to handle unsupervised prediction of shapes in 2D images.
Once we train our model, we have a 3D shape generator that is capable of creating shapes from
a set of encodings $z \in \mathbb{R}^{201}$.
Thus, our goal is to predict the encoding of the object that is displayed in the image.
We do this by training a neural network with images created by the previously trained PrGAN.
In other words, we create a training set that consists of images synthesized by the PrGAN and
the encodings that generated them.
The neural network is a fully connected one, with 2 hidden layers, each one with 512 neurons.
The input of the network is an image and the output is an encoding.
The last number of $z$ describes the view and the other 200 describe the shape.
We use these 200 values to retrieve the shape present in the image.
The network is trained with images created by the PrGAN, but we present the results of the network
using the original dataset images as input in Figure \ref{fig:sp}.
This whole process constitutes a completely unsupervised approach to
creating a model to infer a 3D shape from a single image.

\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{0pt}
\begin{tabular}{cccccccc}
\includegraphics[width=.125\linewidth]{fig/airplane/sel0009.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0012.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0007.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0003.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0002.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0004.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0006.png} &
\includegraphics[width=.125\linewidth]{fig/airplane/sel0008.png} \\
\includegraphics[width=.125\linewidth]{fig/car/sel0010.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0005.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0001.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0004.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0002.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0006.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0007.png} &
\includegraphics[width=.125\linewidth]{fig/car/sel0008.png} \\
\includegraphics[width=.125\linewidth]{fig/vase/sel0013.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0003.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0011.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0015.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0001.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0014.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0016.png} &
\includegraphics[width=.125\linewidth]{fig/vase/sel0007.png} \\
\includegraphics[width=.125\linewidth]{fig/bike/sel0006.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0005.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0008.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0004.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0007.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0003.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0002.png} &
\includegraphics[width=.125\linewidth]{fig/bike/sel0001.png} 
\end{tabular}
\caption{\label{fig:example-samples} A variety of 3D results generated by our PrGAN model trained on 2D views of (from the top row to the bottom row) airplanes, cars, vases, and bikes. These examples are chosen from the gallery images in Fig.~\ref{fig:generate-shapes}}\end{figure*}

